TaskTorrent: a Lightweight Distributed Task-Based Runtime System in C++

We present TaskTorrent, a lightweight distributed task-based runtime in C++. TaskTorrent uses a parametrized task graph to express the task DAG, and one-sided active messages to trigger remote tasks asynchronously. As a result the task DAG is completely distributed and discovered in parallel. It is a C++14 library and only depends on MPI. We explain the API and the implementation. We perform a series of benchmarks against StarPU and ScaLAPACK. Micro benchmarks show it has a minimal overhead compared to other solutions. We then apply it to two large linear algebra problems. TaskTorrent scales very well to thousands of cores, exhibiting good weak and strong scalings.

==> sparse_cholesky.tex <==
\subsection{Sparse cholesky}

\begin{figure}
  \centering
  \subfloat[TaskTorrent strong scalings]{
    \begin{tikzpicture}
      \begin{loglogaxis}[
         xlabel={Cores},xtick={1,4,16,64,256,1024},xticklabels={1,4,16,64,256,1024},
         ylabel={Time [sec.]},width=6cm,legend entries={1,2,4,8,16,32},legend pos=outer north east,ymin=10,
        ]
        \addplot+[] table[x=n_threads_total,y=total_time,discard if not={n_ranks}{1}] {sparse_cholesky/strong_scalings.dat};
        \addplot+[] table[x=n_threads_total,y=total_time,discard if not={n_ranks}{2}] {sparse_cholesky/strong_scalings.dat};
        \addplot+[] table[x=n_threads_total,y=total_time,discard if not={n_ranks}{4}] {sparse_cholesky/strong_scalings.dat};
        \addplot+[] table[x=n_threads_total,y=total_time,discard if not={n_ranks}{8}] {sparse_cholesky/strong_scalings.dat};
        \addplot+[] table[x=n_threads_total,y=total_time,discard if not={n_ranks}{16}] {sparse_cholesky/strong_scalings.dat};
        \addplot+[] table[x=n_threads_total,y=total_time,discard if not={n_ranks}{32}] {sparse_cholesky/strong_scalings.dat};
        \addplot+[dotted,no marks,domain=1:1024] (x,1000/x);
      \end{loglogaxis}
    \end{tikzpicture}
  }
  \subfloat[TaskTorrent weak scalings]{
    \begin{tikzpicture}
      \begin{loglogaxis}[
         xlabel={Cores},xtick={1,4,16,64,256,1024},xticklabels={1,4,16,64,256,1024},
         ylabel={Time [sec.]},width=6cm,ymin=0.5,
        ]
        % \addplot+[black,only marks] table[x=n_ranks,y=total_time] {sparse_cholesky/scalings.dat};
        \addplot+[dashed] table[x=n_threads_total,y=total_time,discard if not={nrows}{262144}] {sparse_cholesky/scalings.dat};
        \addplot+[dashed] table[x=n_threads_total,y=total_time,discard if not={nrows}{512000}] {sparse_cholesky/scalings.dat};
        \addplot+[dashed] table[x=n_threads_total,y=total_time,discard if not={nrows}{1030301}] {sparse_cholesky/scalings.dat};
        \addplot+[dashed] table[x=n_threads_total,y=total_time,discard if not={nrows}{2097152}] {sparse_cholesky/scalings.dat};
        \addplot+[dashed] table[x=n_threads_total,y=total_time,discard if not={nrows}{4173281}] {sparse_cholesky/scalings.dat};
        \addplot+[dotted,no marks,domain=1:32] (x,100/x);
      \end{loglogaxis}
    \end{tikzpicture}
  }
  \caption{Sparse cholesky scalings}
  \label{fig:sparse_cholesky_scalings}
\end{figure}

See \autoref{fig:sparse_cholesky_scalings}
